Exponentials as Substitutions and the Cost of Cut Elimination in Linear Logic

This paper introduces the exponential substitution calculus (ESC), a new presentation of cut elimination for IMELL, based on proof terms and building on the idea that exponentials can be seen as explicit substitutions. The idea in itself is not new, but here it is pushed to a new level, inspired by Accattoli and Kesner's linear substitution calculus (LSC). One of the key properties of the LSC is that it naturally models the sub-term property of abstract machines, that is the key ingredient for the study of reasonable time cost models for the $\lambda$-calculus. The new ESC is then used to design a cut elimination strategy with the sub-term property, providing the first polynomial cost model for cut elimination with unconstrained exponentials. For the ESC, we also prove untyped confluence and typed strong normalization, showing that it is an alternative to proof nets for an advanced study of cut elimination.

==> proofs/confluence/local-commutation.tex <==
% !TEX root = ../../main.tex
\begin{proof}
Let $a \in \set{\axmtwo,\axmone,\tens,\lolli,\axesym,\bang,\axetwo,\baxsym,\bdersym,\bwsym}$, $\tm_{0} \Rew{a} \tm_{1}$ and $\tm_{0} \Rew{a} \tm_{2}$. The proof is by induction on $\tm_{0} \Rew{a} \tm_{1}$, that is, by induction on the context $\ctx$ closing the top level rule $\rootRew{a}$, and case analysis of $\tm_{0} \Rew{a} \tm_{2}$. We deal with each top level case. The inductive cases are treated all in the same way after the top level cases. The top level cases are:
\begin{itemize}
	%%%%%%%%%%%%%%
	\item $\rtoaxmtwo$. We have $\tm_{0} = \cuta{\lctxp\mvartwo}\mvar\tmtwo  \rtoaxmtwo  \lctxp{\cutsub\mvartwo\mvar\tmtwo} = \tm_{1}$. 
	If the second step takes place entirely in $\lctx$ then two steps are independent and the diagram closes in one step on both sides. 

	If the second step takes place in $\tmtwo$, \ie $\tmtwo \Rew{b} \tmtwo'$ then the diagram closes in one step on both sides because by \reflemmap{substitutivity-of-red}{one} we have $\cutsub\mvartwo\mvar\tmtwo \Rew{b} \cutsub\mvartwo\mvar\tmtwo'$, and so:
	\[\begin{array}{cccccc}
\cuta{\lctxp\mvartwo}\mvar\tmtwo 
& \rtoaxmtwo &
\lctxp{\cutsub\mvartwo\mvar\tmtwo}
\\
\downarrow_{b} & &\downarrow_{b}
\\
\cuta{\lctxp\mvartwo}\mvar\tmtwo' 
& \rtoaxmtwo &
\lctxp{\cutsub\mvartwo\mvar\tmtwo'}
\end{array}\]
If the second step involves both $\lctx$ and $\mvartwo$ then it is a $\toaxmone$ step and $\lctx = \lctxtwop{\cuta{\lctxthreep\mval}\mvartwo\lctxfour}$:
	\[\begin{array}{cccccc}
\cuta{\lctxtwop{\cuta{\lctxthreep\mval}\mvartwo\lctxfourp\mvartwo}}\mvar\tmtwo  
&& \rtoaxmtwo &&
\lctxtwop{ \cuta{\lctxthreep\mval}\mvartwo\lctxfourp{ \cutsub\mvartwo\mvar\tmtwo  }}
\\
\downarrow_{\axmone} & &&&\downarrow_{\axmone}
\\
\cuta{\lctxtwop{\lctxthreep{\lctxfourp\mval}}}\mvar\tmtwo  
& \rtoaxmone   &
\lctxtwop{\lctxthreep{\lctxfourp{\cutsub\mval\mvar\tmtwo  }}} 
&
= 
&
\lctxtwop{ \lctxthreep{\cutsub\mvarthree\mvartwo\lctxfourp{ \cutsub\mvartwo\mvar\tmtwo  }}}
\end{array}\]

	%%%%%%%%%%%%%%
	\item $\rtoaxmone$. We have $\tm_{0} = \cuta{\lctxp\mval}\mvar\wctxfp\mvar  \rtoaxmone  \lctxp{\wctxfp\mval} = \tm_{1}$. 
		If the second step takes place entirely in $\lctx$ or entirely in $\mval$ then the diagram closes in one step on both sides. 
		
	If the second step takes place in $\wctxfp\mvar$, \ie $\wctxfp\mvar \Rew{b}\tmtwo$ then the diagram closes in one step on both sides because by \reflemmap{substitutivity-of-red}{two} we have $\tmtwo = \wctxtwofp\mvar$ and $\wctxfp\mval \Rew{b}\wctxtwofp\mval$ and so:
	\[\begin{array}{cccccc}
\cuta{\lctxp\mval}\mvar\wctxfp\mvar 
& \rtoaxmone &
\lctxp{\wctxfp\mval}
\\
\downarrow_{b} & &\downarrow_{b}
\\
\cuta{\lctxp\mval}\mvar\wctxtwofp\mvar 
& \rtoaxmone &
\lctxp{\wctxtwofp\mval}
\end{array}\]
If the second step involves both $\lctx$ and $\mval$ then $\lctxp\mval \Rew{b} \lctxtwop\mvaltwo$ and by \reflemmap{loc-confluence-aux}{four} we have:
	\[\begin{array}{cccccc}
\cuta{\lctxp\mval}\mvar\wctxfp\mvar 
& \rtoaxmone &
\lctxp{\wctxfp\mval}
\\
\downarrow_{b} & &\downarrow_{b}
\\
\cuta{\lctxtwop\mvaltwo}\mvar\wctxfp\mvar 
& \rtoaxmone &
\lctxtwop{\wctxfp\mvaltwo}
\end{array}\]	
	%%%%%%%%%%%%%%
	\item $\rtotens$. We have $\tm_{0} = \cuta{\lctxp{\pair\tmtwo\tmthree}}\mvar \wctxp{\subpar\mvar{\var,\vartwo}\tmfour}
 \rtotens  
\lctxp{\cuta\tmtwo\var \cuta\tmthree\vartwo \wctxp{\tmfour} } = \tm_{1}$. If the second step takes place entirely in $\lctx$, in $\tmtwo$, or in $\tmthree$ then the diagram closes in one step on both sides. 

If the second step takes place in $\wctxp{\subpar\mvar{\var,\vartwo}\tmfour}$ then by \reflemmap{loc-confluence-aux}{one} $\wctxp{\subpar\mvar{\var,\vartwo}\tmfour} \Rew{b} \wctxtwop{\subpar\mvar{\var,\vartwo}\tmfour'}$ with $\wctxp{\tmfour} \Rew{b} \wctxtwop{\tmfour'}$, and so:
\[\begin{array}{cccccc}
\cuta{\lctxp{\pair\tmtwo\tmthree}}\mvar \wctxp{\subpar\mvar{\var,\vartwo}\tmfour}
& \rtotens &
\lctxp{\cuta\tmtwo\var \cuta\tmthree\vartwo \wctxp{\tmfour} }
\\
\downarrow_{b} &&\downarrow_{b}
\\
\cuta{\lctxp{\pair\tmtwo\tmthree}}\mvar \wctxtwop{\subpar\mvar{\var,\vartwo}\tmfour'}
& \rtotens  &
\lctxp{\cuta\tmtwo\var \cuta\tmthree\vartwo \wctxtwop{\tmfour'} }
\end{array}\]
If the second step involves $\lctx$ and $\pair\tmtwo\tmthree$ there are two cases. If the step does not generate a substitution on potentially many variables (\ie it is not $\toaxe$ nor a $\tobang$ step), then it interacts with only either $\tmtwo$ or $\tmthree$, say it has the shape $\lctxp{\pair\tmtwo\tmthree} \Rew{b} \lctxtwop{\pair{\tmtwo'}\tmthree}$ with $b\in\set{\axmtwo,\axmone,\tens,\lolli,\baxsym,\axetwo,\bdersym,\bwsym}$. Then by \reflemmap{loc-confluence-aux}{five} we have the following diagram:  
\[\begin{array}{cccccc}
\cuta{\lctxp{\pair\tmtwo\tmthree}}\mvar \wctxp{\subpar\mvar{\var,\vartwo}\tmfour}
& \rtotens &
\lctxp{\cuta\tmtwo\var \cuta\tmthree\vartwo \wctxp{\tmfour} }
\\
\downarrow_{b} &&\downarrow_{b}
\\
\cuta{\lctxtwop{\pair{\tmtwo'}\tmthree}}\mvar \wctxp{\subpar\mvar{\var,\vartwo}\tmfour}
& \rtotens  &
\lctxtwop{\cuta{\tmtwo'}\var \cuta\tmthree\vartwo \wctxp{\tmfour} }
\end{array}\]
If the reduction instead involves $\tmthree$ one obtain a similar diagram. If instead the step generates a substitution $\cutsub\cdot\evar$, we have:
\[\begin{array}{cccccc}
\cuta{\lctxp{\pair\tmtwo\tmthree}}\mvar \wctxp{\subpar\mvar{\var,\vartwo}\tmfour}
& \rtotens &
\lctxp{\cuta\tmtwo\var \cuta\tmthree\vartwo \wctxp{\tmfour} }
\\
\downarrow_{b} &&\downarrow_{b}
\\
\cuta{\lctxtwop{\pair{\cutsub\cdot\evar\tmtwo}{\cutsub\cdot\evar\tmthree}}}\mvar \wctxp{\subpar\mvar{\var,\vartwo}\tmfour}
& \rtotens  &
\lctxtwop{\cuta{\cutsub\cdot\evar\tmtwo}\var \cuta{\cutsub\cdot\evar\tmthree}\vartwo \wctxp{\tmfour} }
\end{array}\]
where we used the fact that $\evar$ does not occur in $\wctxp{\tmfour}$.
%%%%%%%%%%%
\item $\rtololli$. We have $\tm_{0} = \cuta{\lctxp{\la\vartwo\tmthree}}\mvar \wctxp{\subapp\mvar{\tmtwo,\var} \tmfour}
 \rtololli  
\lctxp{\wctxp{ \cuta\tmtwo\vartwo \cuta\tmthree\var \tmfour }}
 = \tm_{1}$. If the second step takes place entirely in $\lctx$, in $\tmtwo$, in $\tmthree$, or in $\tmfour$ then the diagram closes in one step on both sides. 

If the second step takes place in $\wctxp{\subapp\mvar{\tmtwo,\var} \tmfour}$ then by \reflemmap{loc-confluence-aux}{two} $\wctxp{\subapp\mvar{\tmtwo,\var} \tmfour} \tololli \wctxtwop{\subapp\mvar{\tmtwo',\var} \tmfour'}$ with ($\wctxp{\tmfour} \Rew{b} \wctxtwop{\tmfour'}$ and $\tmtwo' = \tmtwo$) or ($\wctxp{\tmtwo} \Rew{b} \wctxtwop{\tmtwo'}$ and $\tmfour = \tmfour'$), and so either:
\[\begin{array}{cccccc}
\cuta{\lctxp{\la\vartwo\tmthree}}\mvar \wctxp{\subapp\mvar{\tmtwo,\var} \tmfour}
& \rtololli &
\lctxp{\wctxp{ \cuta\tmtwo\vartwo \cuta\tmthree\var \tmfour }}
\\
\downarrow_{b} &&\downarrow_{b}
\\
\cuta{\lctxp{\la\vartwo\tmthree}}\mvar \wctxtwop{\subapp\mvar{\tmtwo,\var} \tmfour'}
& \rtololli  &
\lctxp{\wctxtwop{ \cuta\tmtwo\vartwo \cuta\tmthree\var \tmfour' }}
\end{array}\]
or the same diagram where instead reduction involves $\tmthree$.

If the second step involves both $\lctx$ and $\la\vartwo\tmthree$ then $\lctxp{\la\vartwo\tmthree} \Rew{b} \lctxtwop{\la\vartwo\tmthree'}$. If the step does not generate a substitution on potentially many variables (\ie it is not $\toaxe$ nor a $\tobang$ step). Then by \reflemmap{loc-confluence-aux}{five} we have the following diagram:  
\[\begin{array}{cccccc}
\cuta{\lctxp{\la\vartwo\tmthree}}\mvar \wctxp{\subapp\mvar{\tmtwo,\var} \tmfour}
& \rtololli &
\lctxp{\wctxp{ \cuta\tmtwo\vartwo \cuta\tmthree\var \tmfour }}
\\
\downarrow_{b} &&\downarrow_{b}
\\
\cuta{\lctxtwop{\la\vartwo\tmthree'}}\mvar \wctxp{\subapp\mvar{\tmtwo,\var} \tmfour}
& \rtololli  &
\lctxtwop{\wctxp{ \cuta\tmtwo\vartwo \cuta{\tmthree'}\var \tmfour }}
\end{array}\]

%%%%%%%%%%%%%%
	\item $\rtoaxe$.  We have $\tm_{0} = \cuta{\lctxp\evartwo}\evar\tmtwo  \rtoaxe  \lctxp{\cutsub\evartwo\evar\tmtwo} = \tm_{1}$. 
	If the second step takes place entirely in $\lctx$ then two steps are independent and the diagram closes in one step on both sides. 

	If the second step takes place in $\tmtwo$, \ie $\tmtwo \Rew{b} \tmtwo'$ then the diagram closes in one step on both sides because by \reflemmap{substitutivity-of-red}{one} we have $\cutsub\evartwo\evar\tmtwo \Rew{b} \cutsub\evartwo\evar\tmtwo'$, and so:
	\[\begin{array}{cccccc}
\cuta{\lctxp\evartwo}\evar\tmtwo 
& \rtoaxmtwo &
\lctxp{\cutsub\evartwo\evar\tmtwo}
\\
\downarrow_{b} & &\downarrow_{b}
\\
\cuta{\lctxp\evartwo}\evar\tmtwo' 
& \rtoaxmtwo &
\lctxp{\cutsub\evartwo\evar\tmtwo'}
\end{array}\]
If the second step involves both $\lctx$ and $\evartwo$ then it is a $\tobang$ step of shape $\lctxp\evartwo \tobang \lctxtwop{\bang\tmthree}$. Then:
\[\begin{array}{cccccc}
\cuta{\lctxp\evartwo}\evar\tmtwo 
& \rtoaxe &
\lctxp{\cutsub\evartwo\evar\tmtwo}
\\
 & &\downarrow_{\bang}
\\
\downarrow_{\bang}&&\lctxp{\cutsub{\bang\tmthree}\evartwo\cutsub\evartwo\evar\tmtwo'}
\\
&&=\\
\cuta{\lctxtwop{\bang\tmthree}}\evar\tmtwo' 
& \rtobang &
\lctxp{\cutsub{\bang\tmthree}\evar\tmtwo'}
\end{array}\]	
%%%%%%%%%%%%%%%%%%%%%
	\item $\rtobang$.  We have $\tm_{0} = \cuta{\lctxp{\bang\tmtwo}}\evar \tmthree
 \rtobang  
\lctxp{\cutsub{\bang\tmtwo}\evar\tmthree}
 = \tm_{1}$. If the second step takes place entirely in $\lctx$ then the diagram closes in one step on both sides. 
 
 If the second step takes place in $\tmthree$ then by \reflemmap{substitutivity-of-red}{four} $\cutsub{\bang\tmtwo}\evar\tmthree \tobang \cutsub{\bang\tmtwo}\evar\tmthree'$, and so 
 	\[\begin{array}{cccccc}
\cuta{\lctxp{\bang\tmtwo}}\evar\tmthree 
& \rtobang &
\lctxp{\cutsub{\bang\tmtwo}\evar\tmthree}
\\
\downarrow_{\bang} & &\downarrow_{\bang}
\\
\cuta{\lctxp{\bang\tmtwo}}\evar\tmthree' 
& \rtobang &
\lctxp{\cutsub{\bang\tmtwo}\evar\tmthree'}
\end{array}\]
 If the second step takes place in $\tmtwo$ then by \reflemmap{substitutivity-of-red}{fourb} $\cutsub{\bang\tmtwo}\evar\tmthree \tobang^{*} \cutsub{\bang\tmtwo'}\evar\tmthree$, and so 
 	\[\begin{array}{cccccc}
\cuta{\lctxp{\bang\tmtwo}}\evar\tmthree 
& \rtobang &
\lctxp{\cutsub{\bang\tmtwo}\evar\tmthree}
\\
\downarrow_{\bang} & &\downarrow_{\bang*}
\\
\cuta{\lctxp{\bang\tmtwo'}}\evar\tmthree 
& \rtobang &
\lctxp{\cutsub{\bang\tmtwo'}\evar\tmthree}
\end{array}\]
This diagram is the reason why $\tobang$ is not diamond but only locally confluent.

If the second step involves both $\lctx$ and $\bang\tmtwo$ then $\lctx = \lctxtwop{\cuta{\lctxthreep{\bang\tmtwo'}}\evartwo\lctxfour}$. Then: 
\[\begin{array}{cccccc}
\cuta{\lctxtwop{\cuta{\lctxthreep{\bang\tmtwo'}}\evartwo\lctxfourp{\bang\tmtwo} }}\evar\tmthree 
& \rtobang &
\lctxtwop{\cuta{\lctxthreep{\bang\tmtwo'}}\evartwo\lctxfourp{\cutsub{\bang\tmtwo}\evar\tmthree}} 
\\
 & &\downarrow_{\bang}
\\ 
\downarrow_{\bang}&& \lctxtwop{\lctxthreep{(\cutsub{\bang\tmtwo'}\evartwo\lctxfour)\ctxholep{\cutsub{\bang\tmtwo'}\evartwo\cutsub{\bang\tmtwo}\evar\tmthree}} }
\\
&&=_{\reflemmaeqp{bang-subs-prop}{two}}
\\
\cuta{\lctxtwop{\lctxthreep{(\cutsub{\bang\tmtwo'}\evartwo\lctxfour)\ctxholep{\bang\cutsub{\bang\tmtwo'}\evartwo\tmtwo}}}}\evar\tmthree 

& \rtobang &
\lctxtwop{\lctxthreep{(\cutsub{\bang\tmtwo'}\evartwo\lctxfour)\ctxholep{\cutsub{\bang\cutsub{\bang\tmtwo'}\evartwo\tmtwo}\evar\tmthree}}}  
\end{array}\]
where in the equality we also used the fact that $\evartwo\notin\fv\tmthree$.

%%%%%%%%%%%%%
	\item $\rtobax$.  We have $\tm_{0} =  \cuta{\lctxp{\exval}} \evar \ctxfp{\evar}
 \rtobax 
\lctxp{\cuta{\exval}\evar\ctxfp{\exval}}
 = \tm_{1}$. If the second step takes place entirely in $\lctx$, or in $\ctx$ without duplicating the occurrence of $\evar$ isolated by $\ctx$, then the diagram closes in one step on both sides. 

If the second steps duplicates the occurrence of $\evar$ then $\ctxfp\evar = \ctxtwop{\cuta{\lctxtwop{\evar}} \evartwo \ctxthreefp{\evartwo}}$ and the diagram closes as follows:
	\[\begin{array}{cccccc}
\cuta{\lctxp{\exval}} \evar \ctxtwop{\cuta{\lctxtwop{\evar}} \evartwo \ctxthreefp{\evartwo}}
& \rtobax &
\lctxp{\cuta{\exval} \evar \ctxtwop{\cuta{\lctxtwop{\exval}} \evartwo \ctxthreefp{\evartwo}}}
\\
 & &\downarrow_{\baxsym}
\\
\downarrow_{\baxsym}
&&
\lctxp{\cuta{\exval} \evar \ctxtwop{\lctxtwop{\cuta{\exval} \evartwo \ctxthreefp{\exval}}}}
\\
&&\uparrow_{\baxsym}\\
\cuta{\lctxp{\exval}} \evar \ctxtwop{\lctxtwop{\cuta{\evar} \evartwo \ctxthreefp{\evar}}}
& \rtobax &
\lctxp{\cuta{\exval} \evar \ctxtwop{\lctxtwop{\cuta{\exval} \evartwo \ctxthreefp{\evar}}}}
\end{array}\]
Note that this diagram is not diamond.

If the second step involves both $\lctx$ and $\exval$ then $\exval =\ctxtwofp\evartwo$ and $\lctx = \lctxtwop{\cuta{\lctxthreep{\exval'}}\evartwo\lctxfour}$. Then:
	\[\begin{array}{cccccc}
\cuta{\lctxtwop{\cuta{\lctxthreep{\exval'}}\evartwo\lctxfourp{\ctxtwofp\evartwo}}}\evar \ctxfp\evar
& \rtobax &
\lctxtwop{\cuta{\lctxthreep{\exval'}}\evartwo\lctxfourp{\cuta{\ctxtwofp\evartwo}\evar \ctxfp{\ctxtwofp\evartwo}}}
\\
 &&\downarrow_{\baxsym}
\\ 
\downarrow_{\baxsym}& & 
\lctxtwop{\lctxthreep{\cuta{\exval'}\evartwo\lctxfourp{\cuta{\ctxtwofp{\exval'}}\evar \ctxfp{\ctxtwofp{\evartwo}}}}}

\\
&&\downarrow_{\baxsym}
\\
\cuta{\lctxtwop{\lctxthreep{\cuta{\exval'}\evartwo\lctxfourp{\ctxtwofp{\exval'}}}}}\evar \ctxfp\evar
& \rtobax    &
\lctxtwop{\lctxthreep{\cuta{\exval'}\evartwo\lctxfourp{\cuta{\ctxtwofp{\exval'}}\evar \ctxfp{\ctxtwofp{\exval'}}}}}
\end{array}\]
Note that this diagram is not diamond.

%%%%%%%%%%%%%
	\item $\rtoaxetwo$.  We have $\tm_{0} =  \cuta{\lctxp{\evartwo}}\evar\ctxp{\dera\evar\var \tmtwo}
 \rtoaxetwo 
\lctxp{\cuta{\evartwo}\evar\ctxp{\dera\evartwo\var \tmtwo}}
 = \tm_{1}$. If the second step takes place entirely in $\lctx$, or in $\ctx$ without duplicating the occurrence of $\evar$ isolated by $\ctx$, then the diagram closes in one step on both sides. 

If the second steps takes place in $\ctxp{\dera\evar\var \tmtwo}$ then by \reflemmap{loc-confluence-aux}{three} the reduct is $\ctxtwop{\dera\evar\var \tmtwo'}$ and the diagram closes as follows:
\[\begin{array}{cccccc}
\cuta{\lctxp{\evartwo}}\evar\ctxp{\dera\evar\var \tmtwo}
& \rtoaxetwo &
\lctxp{\cuta{\evartwo}\evar\ctxp{\dera\evartwo\var \tmtwo}}
\\
\downarrow_{\axetwo} & &\downarrow_{\axetwo}
\\
\cuta{\lctxp{\evartwo}}\evar\ctxtwop{\dera\evar\var \tmtwo'}
& \rtoaxetwo &
\lctxp{\cuta{\evartwo}\evar\ctxtwop{\dera\evartwo\var \tmtwo'}}
\end{array}\]
Note that the second step cannot involve $\lctx$ and $\evartwo$.

%%%%%%%%%%%%%
	\item $\rtobder$.  We have $\tm_{0} =  \cuta{\lctxp{\bang\tmtwo}}\evar\ctxp{\dera\evar\var \tmthree}
 \rtobder 
\lctxp{\cuta{\bang\tmtwo}\evar\ctxp{\cuta\tmtwo\var \tmthree}}
 = \tm_{1}$. If the second step takes place entirely in $\lctx$, or in $\ctx$ without duplicating the dereliction on $\evar$ isolated by $\ctx$, then the diagram closes in one step on both sides. 

If the second steps duplicates the dereliction on $\evar$ then $\ctx = \ctxtwop{\cuta{\lctxtwop{\bang\ctxthree}} \evartwo \ctxfourp{\dera\evartwo\vartwo\tmfour}}$ and the diagram closes as follows:
		\[\small\begin{array}{cccccc}
\cuta{\lctxp{{\bang\tmtwo}}} \evar \ctxtwop{\cuta{\lctxtwop{\bang\ctxthreep{\dera\evar\var \tmthree}}} \evartwo \ctxfourp{\dera\evartwo\vartwo\tmfour}}
& \rtobder &
\lctxp{\cuta{{\bang\tmtwo}} \evar \ctxtwop{\cuta{\lctxtwop{\bang\ctxthreep{\cuta\tmtwo\var \tmthree}}} \evartwo \ctxthreefp{\dera\evartwo\vartwo\tmfour}}}
\\
 & &\downarrow_{\bdersym}
\\
\downarrow_{\bdersym}
&&
\lctxp{\cuta{{\bang\tmtwo}} \evar \ctxtwop{\lctxtwop{\cuta{\bang\ctxthreep{\cuta\tmtwo\var \tmthree}}} \evartwo \ctxfourp{\cuta{\bang\ctxthreep{\cuta\tmtwo\var \tmthree}}\vartwo\tmfour}}}
\\
&&\uparrow_{\bdersym}\\
\cuta{\lctxp{{\bang\tmtwo}}} \evar \ctxtwop{\lctxtwop{\cuta{\bang\ctxthreep{\dera\evar\var \tmthree}}} \evartwo \ctxfourp{\cuta{\bang\ctxthreep{\dera\evar\var \tmthree}}\vartwo\tmfour}}
& \rtobder &
\lctxp{\cuta{{\bang\tmtwo}} \evar \ctxtwop{\lctxtwop{\cuta{\bang\ctxthreep{\cuta\tmtwo\var \tmthree}}} \evartwo \ctxfourp{\cuta{\bang\ctxthreep{\dera\evar\var \tmthree}}\vartwo\tmfour}}}
\end{array}\]
Note that this diagram is not diamond.

If the second step involves both $\lctx$ and $\bang\tmtwo$ then $\tmtwo=\ctxtwop{\dera\evartwo\vartwo\tmfour}$ and $\lctx = \lctxtwop{\cuta{\lctxthreep{\bang\tmfive}}\evartwo\lctxfour}$. Then:
	\[\small\begin{array}{cccccc}
\cuta{\lctxtwop{\cuta{\lctxthreep{\bang\tmfive}}\evartwo\lctxfourp{\bang\ctxtwop{\dera\evartwo\vartwo\tmfour}}}}\evar \ctxp{\dera\evar\var \tmthree}
& \rtobder &
\lctxtwop{\cuta{\lctxthreep{\bang\tmfive}}\evartwo\lctxfourp{\cuta{\bang\ctxtwop{\dera\evartwo\vartwo\tmfour}}\evar \ctxp{\cuta{\ctxtwop{\dera\evartwo\vartwo\tmfour}}\var \tmthree}}}
\\
 &&\downarrow_{\bdersym}
\\ 
\downarrow_{\bdersym}&&\lctxtwop{\lctxthreep{\cuta{\bang\tmfive}\evartwo\lctxfourp{\cuta{\bang\ctxtwop{\cuta{\tmfive}\vartwo\tmfour}}\evar \ctxp{\cuta{\ctxtwop{\dera\evartwo\vartwo\tmfour}}\var \tmthree}}}}

\\
&&\downarrow_{\bdersym}
\\
\cuta{\lctxtwop{\lctxthreep{\cuta{\bang\tmfive}\evartwo\lctxfourp{\bang\ctxtwop{\cuta{\tmfive}\vartwo\tmfour}}}}}\evar \ctxp{\dera\evar\var \tmthree}
& \rtobder   &
\lctxtwop{\lctxthreep{\cuta{\bang\tmfive}\evartwo\lctxfourp{\cuta{\bang\ctxtwop{\cuta{\tmfive}\vartwo\tmfour}}\evar \ctxp{\cuta{\ctxtwop{\cuta{\tmfive}\vartwo\tmfour}}\var \tmthree}}}}
\end{array}\]
Note that this diagram is not diamond.

%%%%%%%%%%%%%
	\item $\rtobw$.  We have $\tm_{0} =  \cuta{\lctxp{\exval}}\evar \tmtwo
 \rtobw  
\lctxp{\tmtwo}
 = \tm_{1}$ with $\evar\notin\fv\tmtwo$. If the second step takes place entirely in $\lctx$ or $\tmtwo$, then the diagram closes in one step on both sides. If the step takes place in $\exval$ then the diagram is
\[\begin{array}{cccccc}
\cuta{\lctxp{\exval}}\evar \tmtwo
& \rtobw &
\lctxp{\tmtwo}
\\
\downarrow_{\bwsym} & &=
\\
\cuta{\lctxp{\exval'}}\evar \tmtwo
& \rtobw &
\lctxp{\tmtwo}
\end{array}\]
Note that the diagram is not diamond.
\end{itemize}

%%%%%%%%%%%%%
Now, the inductive cases:
\begin{itemize}
	\item \emph{Inductive cases different from cut}: these cases all go in the same way. We spell out the one for tensor. Let $\tm_{0} = \pair\tmtwo\tmthree \Rew{a} \pair{\tmtwo'}\tmthree = \tm_{1}$. If the second step is in $\tmtwo$ then the statement follows from the \ih, otherwise it is in $\tmthree$ and the two steps are disjoint and the diagram closes in one step on both sides.
	
	\item \emph{Inductive case left of cut}: $\tm_{0} = \cuta\tmtwo\var\tmthree \Rew{a}\cuta{\tmtwo'}\var\tmthree = \tm_{1}$. If the second step is in $\tmtwo$ we use the \ih, and if it is in $\tmthree$ then the two steps are disjoint. The last possibility is that the external cut itself if a $\Rew{a}$ redex. But then we are again in a top level case, which is treated by simply switching the role of the two steps.
	
		\item \emph{Inductive case right of cut}: $\tm_{0} = \cuta\tmtwo\var\tmthree \Rew{a}\cuta{\tmtwo}\var{\tmthree'} = \tm_{1}$. If the second step is in $\tmthree$ we use the \ih, and if it is in $\tmtwo$ then the two steps are disjoint. The last possibility is that the external cut itself if a $\Rew{a}$ redex. But then we are again in a top level case, which is treated by simply switching the role of the two steps.
\end{itemize}
\end{proof}

==> proofs/confluence/local-confluence-exp-small.tex <==
% !TEX root = ../../main.tex
The proof follows the same structure as for $\tom$. We treat the root cases, the inductive cases follow from the root ones and the \ih, exactly as for $\tom$.  We have $\tm_{0} = \cuta{\exval}\evar \tmthree
 \rtoess  
\cutsub{\exval}\evar\tmthree
 = \tm_{1}$.
 
 If the second $\toess$ takes place in $\tmthree$ then by \reflemmap{substitutivity-of-red}{four} $\cutsub{\exval}\evar\tmthree \toess \cutsub{\exval}\evar\tmthree'$, and so 
 	\[\begin{array}{cccccc}
\cuta{\exval}\evar\tmthree 
& \rtoess &
\cutsub{\exval}\evar\tmthree
\\
\downarrow_{\ess} & &\downarrow_{\ess}
\\
\cuta{\exval}\evar\tmthree' 
& \rtoess &
\cutsub{\exval}\evar\tmthree'
\end{array}\]
 If the second step takes place in $\exval$ then by \reflemmap{substitutivity-of-red}{fourb} $\cutsub{\exval}\evar\tmthree \toess^{*} \cutsub{\exval'}\evar\tmthree$, and so 
 	\[\begin{array}{cccccc}
\cuta{\exval}\evar\tmthree 
& \rtoess &
\cutsub{\exval}\evar\tmthree
\\
\downarrow_{\ess} & &\downarrow_{\ess*}
\\
\cuta{\exval'}\evar\tmthree 
& \rtoess &
\cutsub{\exval'}\evar\tmthree
\end{array}\]
This diagram is the reason why $\toess$ is not diamond but only locally confluent.

%If the second step $\Rew{b}$ involves both $\lctx$ and $\bang\tmtwo$ then it can be both a $\toaxe$ or a $\tobang$ step. If it is a $\tobang$ step then $\lctx = \lctxtwop{\cuta{\lctxthreep{\bang\tmtwo'}}\evartwo\lctxfour}$ and: 
%\[\begin{array}{cccccc}
%\cuta{\lctxtwop{\cuta{\lctxthreep{\bang\tmtwo'}}\evartwo\lctxfourp{\bang\tmtwo} }}\evar\tmthree 
%& \rtobang &
%\lctxtwop{\cuta{\lctxthreep{\bang\tmtwo'}}\evartwo\lctxfourp{\cutsub{\bang\tmtwo}\evar\tmthree}} 
%\\
% & &\downarrow_{\bang}
%\\ 
%\downarrow_{\bang}&& \lctxtwop{\lctxthreep{(\cutsub{\bang\tmtwo'}\evartwo\lctxfour)\ctxholep{\cutsub{\bang\tmtwo'}\evartwo\cutsub{\bang\tmtwo}\evar\tmthree}} }
%\\
%&&=_{\reflemmaeqp{bang-subs-prop}{two}}
%\\
%\cuta{\lctxtwop{\lctxthreep{(\cutsub{\bang\tmtwo'}\evartwo\lctxfour)\ctxholep{\bang\cutsub{\bang\tmtwo'}\evartwo\tmtwo}}}}\evar\tmthree 
%
%& \rtobang &
%\lctxtwop{\lctxthreep{(\cutsub{\bang\tmtwo'}\evartwo\lctxfour)\ctxholep{\cutsub{\bang\cutsub{\bang\tmtwo'}\evartwo\tmtwo}\evar\tmthree}}}  
%\end{array}\]
%where in the equality we also used the fact that $\evartwo\notin\fv\tmthree$.
%
%If $\Rew{b}$ is a $\toaxe$ step then $\lctx = \lctxtwop{\cuta{\lctxthreep{\evarthree}}\evartwo\lctxfour}$ with $\evarthree\in\evars$ and: 
%\[\begin{array}{cccccc}
%\cuta{\lctxtwop{\cuta{\lctxthreep{\evarthree}}\evartwo\lctxfourp{\bang\tmtwo} }}\evar\tmthree 
%& \rtobang &
%\lctxtwop{\cuta{\lctxthreep{\evarthree}}\evartwo\lctxfourp{\cutsub{\bang\tmtwo}\evar\tmthree}} 
%\\
% & &\downarrow_{\axe}
%\\ 
%\downarrow_{\axe}&& \lctxtwop{\lctxthreep{(\cutsub{\evarthree}\evartwo\lctxfour)\ctxholep{\cutsub{\evarthree}\evartwo\cutsub{\bang\tmtwo}\evar\tmthree}} }
%\\
%&&=_{\reflemmaeqp{bang-subs-prop}{two}}
%\\
%\cuta{\lctxtwop{\lctxthreep{(\cutsub{\evarthree}\evartwo\lctxfour)\ctxholep{\bang\cutsub{\evarthree}\evartwo\tmtwo}}}}\evar\tmthree 
%
%& \rtobang &
%\lctxtwop{\lctxthreep{(\cutsub{\evarthree}\evartwo\lctxfour)\ctxholep{\cutsub{\bang\cutsub{\evarthree}\evartwo\tmtwo}\evar\tmthree}}}  
%\end{array}\]
%where in the equality we also used the fact that $\evartwo\notin\fv\tmthree$.


==> proofs/confluence/strong-commutation-micro.tex <==
% !TEX root = ../../main.tex
Let $a \in \set{\axmtwo,\axmone,\tens,\lolli}$, $b \in \set{\axeone,\axetwo,\bder,\wsym}$, $\tm_{0} \Rew{a} \tm_{1}$ and $\tm_{0} \Rew{b} \tm_{2}$. The proof is by induction on $\tm_{0} \Rew{a} \tm_{1}$, that is, by induction on the context $\ctx$ closing the root rule $\rootRew{a}$, and case analysis of $\tm_{0} \Rew{b} \tm_{2}$. We deal with each root case $\rootRew{a}$ for $\Rew{a}$ but also with each root case for $\rootRew{b}$ for $\Rew{b}$, because they are used in the inductive cases for $\Rew{a}$. The inductive cases go as for the strong commutation of $\tom$ and $\toess$. The multiplicative cases go exactly as in the previous point. The remaining root cases are:
\begin{itemize}
	%%%%%%%%%%%%%%%%%%
\item $\rtoaxeone$.   We have $\tm_{0} =  \cuta{\exval} \evar \ctxfp{\evar}
 \rtoaxeone 
\cuta{\exval}\evar\ctxfp{\exval}
 = \tm_{1}$.
If $\Rew{a}$ takes place in $\exval$ then the diagram is:
	\[\begin{array}{cccccc}
 \cuta{\exval} \evar \ctxfp{\evar}
& \rtoaxeone &
\cuta{\exval}\evar\ctxfp{\exval}
\\
 & &\downarrow_{a}
\\
\downarrow_{a} && 
\cuta{\exvaltwo} \evar \ctxfp{\exval}\\
&&\downarrow_{a}\\
\cuta{\exvaltwo} \evar \ctxfp{\evar}
& \rtoaxeone &
\cuta{\exvaltwo}\evar\ctxfp{\exvaltwo}
\end{array}\]
Note that it is not a diamond diagram.

If $\Rew{a}$ takes place in $\ctxfp\evar$ then by \reflemmap{aux-props-loc-confl-strong-comm}{five} we have $\ctxfp\evar \Rew{a} \ctxtwofp\evar$ for a $\ctxtwo$ such that $\ctxfp\exval \Rew{a} \ctxtwofp\exval$. Then we have the following diagram:
	\[\begin{array}{cccccc}
 \cuta{\exval} \evar \ctxfp{\evar}
& \rtoaxeone &
\cuta{\exval}\evar\ctxfp{\exval}
\\
\downarrow_{a} & &\downarrow_{a}
\\
\cuta{\exval} \evar \ctxtwofp{\evar}
& \rtoaxeone &
\cuta{\exval}\evar\ctxtwofp{\exval}
\end{array}\]

%%%%%%%%%%%%%
	\item $\rtoaxetwo$.  We have $\tm_{0} =  \cuta{\evartwo}\evar\ctxp{\dera\evar\var \tmtwo}
 \rtoaxetwo 
\cuta{\evartwo}\evar\ctxp{\dera\evartwo\var \tmtwo}
 = \tm_{1}$. 
If $\Rew{a}$ takes place in $\ctxp{\dera\evar\var \tmtwo}$ then by \reflemmap{aux-props-loc-confl-strong-comm}{six} we have $\ctxp{\dera\evar\var \tmtwo} \Rew{a} \ctxtwop{\dera\evar\var \tmtwo'}$ for $\ctxtwo$ and $\tmtwo'$ such that $\ctxp{\dera\evartwo\var \tmtwo} \Rew{a} \ctxtwop{\dera\evartwo\var \tmtwo'}$. Then we have the following diagram:
\[\begin{array}{cccccc}
\cuta{\evartwo}\evar\ctxp{\dera\evar\var \tmtwo}
& \rtoaxetwo &
\cuta{\evartwo}\evar\ctxp{\dera\evartwo\var \tmtwo}\\
\downarrow_{a} & &\downarrow_{a}
\\
\cuta{\evartwo}\evar \ctxtwop{\dera\evar\var \tmtwo'}
& \rtoaxeone &
\cuta{\evartwo}\evar \ctxtwop{\dera\evartwo\var \tmtwo'}
\end{array}\]

%%%%%%%%%%%%%
	\item $\rtobder$.  We have $\tm_{0} =  \cuta{\bang\tmtwo}\evar\ctxp{\dera\evar\var \tmthree}
 \rtobder 
\cuta{\bang\tmtwo}\evar\ctxp{\lctxp{\cuta\val\var \tmthree}}
 = \tm_{1}$ with $\tmtwo = \lctxp\val$. 
If $\Rew{a}$ takes place in $\tmtwo=\lctxp\val$, that is, $\lctxp\val \Rew{a} \lctxtwop\valtwo=\tmtwo'$ then the diagram is:
	\[\begin{array}{cccccc}
\cuta{\bang\tmtwo}\evar\ctxp{\dera\evar\var \tmthree}
& \rtobder &
\cuta{\bang\tmtwo}\evar\ctxp{\lctxp{\cuta\val\var \tmthree}}\\
 & &\downarrow_{a} 
\\
\downarrow_{a} && 
\cuta{\bang\tmtwo'}\evar\ctxp{\lctxp{\cuta{\val}\var \tmthree}}
\\
&&\downarrow_{a} (\reflemmaeqp{deformations}{split})\\
\cuta{\bang\tmtwo'}\evar\ctxp{\dera\evar\var \tmthree}
& \rtoaxeone &
\cuta{\bang\tmtwo'}\evar\ctxp{\lctxtwop{\cuta{\valtwo}\var \tmthree}}\\
\end{array}\]
Note that it is not a diamond diagram.

If $\Rew{a}$ takes place in $\ctxp{\dera\evar\var \tmthree}$ then by \reflemmap{aux-props-loc-confl-strong-comm}{six} we have $\ctxp{\dera\evar\var \tmthree} \Rew{a} \ctxtwop{\dera\evar\var \tmthree'}$ for $\ctxtwo$ and $\tmtwo'$ such that $\ctxp{\lctxp{\cuta\val\var \tmthree}} \Rew{a} \ctxtwop{\lctxp{\cuta\val\var \tmthree'}}$. Then we have the following diagram:
\[\begin{array}{cccccc}
\cuta{\bang\tmtwo}\evar\ctxp{\dera\evar\var \tmthree}
& \rtobder &
\cuta{\bang\tmtwo}\evar\ctxp{\lctxp{\cuta\val\var \tmthree}}\\
\downarrow_{a} & &\downarrow_{a}
\\
\cuta{\bang\tmtwo}\evar \ctxtwop{\dera\evar\var \tmthree'}
& \rtoaxeone &
\cuta{\bang\tmtwo}\evar\ctxtwop{\lctxp{\cuta\val\var \tmthree'}}
\end{array}\]

%%%%%%%%%%%%%
	\item $\rtobw$.  We have $\tm_{0} =  \cuta{\exval}\evar \tmtwo
 \rtobw  
\tmtwo
 = \tm_{1}$ with $\evar\notin\fv\tmtwo$. If $\Rew{a}$ takes place entirely in $\tmtwo$, then the diagram closes in one step on both sides. If the step takes place in $\exval$ then the diagram is
\[\begin{array}{cccccc}
\cuta{\exval}\evar \tmtwo
& \rtobw &
\tmtwo
\\
\downarrow_{a} & &=
\\
\cuta{\exval'}\evar \tmtwo
& \rtobw &
\tmtwo
\end{array}\]
Note that the diagram is not diamond.
\end{itemize}

==> proofs/confluence/strong-commutation-small.tex <==
% !TEX root = ../../main.tex
Let $a \in \set{\axmtwo,\axmone,\tens,\lolli}$, $\tm_{0} \Rew{a} \tm_{1}$ and $\tm_{0} \toess \tm_{2}$. The proof is by induction on $\tm_{0} \Rew{a} \tm_{1}$, that is, by induction on the context $\ctx$ closing the root rule $\rootRew{a}$, and case analysis of $\tm_{0} \toess \tm_{2}$. We deal with each root case $\rootRew{a}$ for $\Rew{a}$ but also with each root case for $\toess$, because they are used in the inductive cases for $\Rew{a}$. The inductive cases for $\Rew{a}$ are treated all in the same way after both $\rootRew{a}$ and $\rtoess$. The root cases are all exactly as those for local confluence of $\tom$ and $\toess$ in \refprop{loc-confluence}, but for the case of $\toaxmone$, which is simpler, and where clash-freeness does not play a role ($\toaxmone$ is the only place where clash-freeness plays a role in \refprop{loc-confluence}). We spell out the different case:
\begin{itemize}
	%%%%%%%%%%%%%%
	\item $\rtoaxmone$. We have $\tm_{0} = \cuta{\mval}\mvar\mctxfp\mvar  \rtoaxmone  \mctxfp\mval = \tm_{1}$. 
		If $\Rew{b}$ takes place entirely in $\mval$ then the diagram closes in one step on both sides. 

If $\Rew{b}$ takes place in $\mctxfp\mvar$, \ie $\mctxfp\mvar \Rew{b}\tmtwo$ then by \reflemmap{aux-props-loc-confl-strong-comm}{two} there are two mutually exclusive cases:
	\begin{enumerate}
		\item $\tmtwo = \mctxtwofp{\mvar}$ for some 
$\mctxtwo$ such that $\mvar\notin\fv\mctxtwo$ and $\mctxfp\mval \Rew{b} \mctxtwofp\mval$ for every $\mval$. Then:
	\[\begin{array}{cccccc}
\cuta{\mval}\mvar\mctxfp\mvar 
& \rtoaxmone &
\mctxfp\mval
\\
\downarrow_{b} & &\downarrow_{b}
\\
\cuta{\mval}\mvar\mctxtwofp\mvar 
& \rtoaxmone &
\mctxtwofp\mval
\end{array}\]


		\item $\mctx = \mctxtwop{\cuta\ctxhole\mvartwo\tmthree}$ and $\Rew{b}$ reduces the cut on $\mvartwo$. This case is impossible, because by hypothesis $\Rew{b}$ is an exponential step.
		\end{enumerate}
 
%%%%%%%%%%%%%%%
%	\item $\rtoaxmtwo$. Exactly as in the analogous sub-case of multiplicative local confluence (\refpropp{loc-confluence}{mult}), which does not rely on the hypothesis of clash-freeness. 
%
%	%%%%%%%%%%%
%\item $\rtololli$. Exactly as in the analogous sub-case of multiplicative local confluence (\refpropp{loc-confluence}{mult}), which does not rely on the hypothesis of clash-freeness. 
%
%%%%%%%%%%%%%%%%%%%
%\item $\rtoaxe$.  Exactly as in the analogous sub-case of small-step exponential local confluence (\refpropp{loc-confluence}{small-exp}). 
%%%%%%%%%%%%%%%%%%%%%%
%	\item $\rtobang$.  Exactly as in the analogous sub-case of small-step exponential local confluence (\refpropp{loc-confluence}{small-exp}). 
\end{itemize}

%%%%%%%%%%%%%
Now, the inductive cases:
\begin{itemize}
	\item \emph{Inductive cases different from cut}: these cases all go in the same way. We spell out the one for tensor. Let $\tm_{0} = \pair\tmtwo\tmthree \Rew{a} \pair{\tmtwo'}\tmthree = \tm_{1}$. If $\Rew{b}$ is in $\tmtwo$ then the statement follows from the \ih, otherwise $\Rew{b}$ is in $\tmthree$, thus the two steps are disjoint, and the diagram is a one-step commutation diagram.
	
	\item \emph{Inductive case left of cut}: $\tm_{0} = \cuta\tmtwo\var\tmthree \Rew{a}\cuta{\tmtwo'}\var\tmthree = \tm_{1}$. If $\Rew{b}$ is in $\tmtwo$ we use the \ih, and if it is in $\tmthree$ then the two steps are disjoint. The last possibility is that the external cut itself is the $\Rew{b}$ redex. But then we are in a root case for $\Rew{b}$, which has been treated above.
	
		\item \emph{Inductive case right of cut}: $\tm_{0} = \cuta\tmtwo\var\tmthree \Rew{a}\cuta{\tmtwo}\var{\tmthree'} = \tm_{1}$. If $\Rew{b}$ is in $\tmthree$ we use the \ih, and if it is in $\tmtwo$ then the two steps are disjoint. The last possibility is that the external cut itself is the $\Rew{b}$ redex. But then we are in a root case for $\Rew{b}$, which has been treated above.
	\end{itemize}


==> proofs/strategy/deformations.tex <==
% !TEX root = ../../main.tex
\begin{proof}
\hfill
\begin{enumerate}
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\item By induction on the step $\mctxfp\mvar \Rew{a} \tmtwo$.  The top-level multiplicative cases are:
\begin{itemize}
%%%%%%%%%%%%%%
	\item $\rtoaxmone$. We have $\mctxfp\mvar = \cuta{\mvaltwo}\mvartwo\mctxthreefp\mvartwo  \rtoaxmone  \mctxthreefp\mvaltwo = 
\tmtwo$ with $\ctx = \cuta{\mvaltwo}\mvartwo\mctxthree$. We can assume that $\mvaltwo$ is not a variable, because that case is covered by the next top-level case. And so we are not in case $(b)$. Two cases:
\begin{enumerate}
\item \emph{The hole of $\mctx$ is in the left sub-term $\mvaltwo$ of the root cut.} Then $\mctx = \cuta{\mctx^\bullet}\mvartwo\mctxthreefp\mvartwo$ for some $\mctx^\bullet$. The root step then writes as:
	\[\mctxfp\mvar = \cuta{\mctx^\bullet\ctxholefp\mvar}\mvartwo\mctxthreefp\mvartwo  
 \rtoaxmone \mctxthreefp{\mctx^\bullet\ctxholefp\mvar} = \tmtwo\]
Case $(a)$ holds by taking $\mctxtwo \defeq \mctxthreefp{\mctx^\bullet}$, for which we have $\mctxtwofp\mvar = \mctxthreefp{\mctx^\bullet\ctxholefp\mvar}= \tmtwo$ and
\[\mctxfp\mval =
\cuta{\mctx^\bullet\ctxholefp\mval}\mvartwo\mctxthreefp\mvartwo  
 \rtoaxmone \mctxthreefp{\mctx^\bullet\ctxholefp\mval}
 = \mctxtwofp\mval
\]

\emph{Moreover part}. It does not apply, because $\mctx$ is bad (having its hole inside a cut value).


\item \emph{The hole of $\mctx$ is in the right sub-term $\mctxthree$ of the root cut.} Then $\mctx = \cuta{\mvaltwo}\mvartwo\mctxfour$ for some $\mctxthree$ such that $\mctxthreefp\mvartwo = \mctxfourfp\mvar$ and $\mctxthree\parallel \mctxfour$. Then there is double context $\cctx_{\mctxthree, \mctxfour}$ such that $\cctx_{\mctxthree, \mctxfour}\ctxholep{\mvartwo,\cdot} =\mctxfour$ and $\cctx_{\mctxthree, \mctxfour}\ctxholep{\cdot,\mvar} =\mctxthree$. The root step then writes as:
	\[\mctxfp\mvar = \cuta{\mvaltwo}\mvartwo\mctxfourfp\mvar = 
\cuta{\mvaltwo}\mvartwo\cctx_{\mctxthree, \mctxfour}\ctxholefp{\mvartwo,\mval} \rtoaxmone \cctx_{\mctxthree, \mctxfour}\ctxholefp{\mvaltwo,\mvar} = \tmtwo\]
Case $(a)$ holds by taking $\mctxtwo \defeq \cctx_{\mctxthree, \mctxfour}\ctxholep{\mvaltwo,\cdot}$, for which we have $\mctxtwop\mvar = \cctx_{\mctxthree, \mctxfour}\ctxholep{\mvaltwo,\mvar} = \mctxthreep\mvaltwo= \tmtwo$ and
\[\mctxfp\mval =
\cuta{\mvaltwo}\mvartwo\mctxfourfp\mval = 
\cuta{\mvaltwo}\mvartwo\cctx_{\mctxthree, \mctxfour}\ctxholefp{\mvartwo,\mval} \rtoaxmone \cctx_{\mctxthree, \mctxfour}\ctxholefp{\mvaltwo,\mval} = \mctxtwofp\mval
\]

\emph{Moreover part}. If $\ctx=\cuta{\mval}\mvartwo\mctxthree$ and $\mctx = \cuta{\mvaltwo}\mvartwo\mctxfour$ are good then $\mctxfour=\cctx_{\mctxthree, \mctxfour}\ctxholep{\mvartwo,\cdot}$ is good (because $\mctx$ is) and so $\mctxtwo \defeq \cctx_{\mctxthree, \mctxfour}\ctxholep{\mvaltwo,\cdot}$ is good by \reflemma{double-ctx-repl} and with the same dominating free variables. Similarly, the position of the step $\mctxfp\mval \rtoaxmone \mctxtwofp\mval$ is the context $\cuta{\mvaltwo}\mvartwo\cctx_{\mctxthree, \mctxfour}\ctxholefp{\cdot,\mval}$ which is good and with the same dominating free variables because of \reflemma{double-ctx-repl} and the hypothesis that 
$\cuta{\mvaltwo}\mvartwo\cctx_{\mctxthree, \mctxfour}\ctxholep{\cdot,\mvar} =\cuta{\mvaltwo}\mvartwo\mctxthree=\ctx$ is good.
\end{enumerate}


	%%%%%%%%%%%%%%
	\item $\rtoaxmtwo$. We have $\mctxfp\mvar = \cuta{\mvarthree}\mvartwo\mctxthreep{\tm_\mvartwo}  \rtoaxmtwo  \mctxthreep{\tm_\mvarthree} = \tmtwo$ with $\ctx = \cuta{\mvarthree}\mvartwo\mctxthree$ and $\tm_\mvartwo$ is $\mvartwo$, or a par or a subtraction of conclusion $\mvartwo$. Cases:
	\begin{enumerate}
	\item \emph{The hole of $\mctx$ is in the left sub-term $\mvarthree$ of the root cut.} Then $\mvarthree = \mvar$ and $\mctx = \cuta{\ctxhole}\mvartwo\mctxthreep{\tm_\mvartwo}$ then we are in case $(b)$. 
		\item \emph{The hole of $\mctx$ is in the right sub-term $\mctxthreep{\tm_\mvartwo}$ of the root cut}. Then $\mctx = \cuta{\mvarthree}\mvartwo\mctxfour$ for some $\mctxfour$ such that $\mctxfourp\mvar=\mctxthreep{\tm_\mvartwo}$. Two sub-cases:
	\begin{enumerate}
	\item $\mctxthree\parallel\mctxfour$, then this case goes as sub-case $b$ of the $\rtoaxmone$ case (we are in case $(a)$), including the \emph{moreover} part.
	
	\item $\mctxthree\outer\mctxfour$. In this case $\tm_\mvartwo$ cannot be a variable. Therefore, $\mctxfour = \mctxthreep{\cyanbrackets{\mvartwo\cdots}\mctx^\bullet}$ for some $\mctx^\bullet$ and where $\cyanbrackets{\mvartwo\cdots}$ is a par or a subtraction of conclusion $\mvartwo$. The root step then writes as:
	\[\mctxfp\mvar = \cuta{\mvarthree}\mvartwo\mctxthreep{\cyanbrackets{\mvartwo\cdots}\mctx^\bullet\ctxholefp\mvar}  \rtoaxmtwo  \mctxthreep{\cyanbrackets{\mvarthree\cdots}\mctx^\bullet\ctxholefp\mvar} = \tmtwo\]
	Then taking $\mctxtwo \defeq \mctxthreep{\cyanbrackets{\mvarthree\cdots}\mctx^\bullet}$ we have $\tmtwo = \mctxtwofp\mvar$, and
		\[\mctxfp\mval = \cuta{\mvarthree}\mvartwo\mctxthreep{\cyanbrackets{\mvartwo\cdots}\mctx^\bullet\ctxholefp\mval}  \rtoaxmtwo  \mctxthreep{\cyanbrackets{\mvarthree\cdots}\mctx^\bullet\ctxholefp\mval} = \mctxtwofp\mval\]
		
	\emph{Moreover part}. If $\ctx= \cuta{\mvarthree}\mvartwo\mctxthree$ and $\mctx= \cuta{\mvarthree}\mvartwo\mctxthreep{\cyanbrackets{\mvartwo\cdots}\mctx^\bullet}$ are good then $\mctxthreep{\cyanbrackets{\mvartwo\cdots}\mctx^\bullet}$ is good and  $\mvartwo \notin \dfv{\mctxthreep{\cyanbrackets{\mvartwo\cdots}\mctx^\bullet}}$. Then $\mctxtwo=\mctxthreep{\cyanbrackets{\mvarthree\cdots}\mctx^\bullet}$ is good and has the same dominating free variables because of \reflemma{good-stable-by-sub-ren}. The step $\mctxfp\mval   \rtoaxmtwo   \mctxtwofp\mval$ has position $\ctx$, which is good by hypothesis.
	\end{enumerate}
\end{enumerate}

	
%%%%%%%%%%%%%%
	\item $\rtotens$. We have $\mctxfp\mvar = \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo \mctxthreep{\para\mvartwo\var\vartwo \tmfour}
 \rtotens  
 \mctxthreep{ \lctxp{\cuta\val\var \lctxtwop{\cuta\valtwo\vartwo \tmfour}}}  = \tmtwo$ with $\ctx = \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo \mctxthree$. Clearly, it is not case $(b)$, and one shows that we are in case $(a)$. There are two cases.
 \begin{enumerate}
	\item \emph{The hole of $\mctx$ is in the left sub-term $\pair{\lctxp\val}{\lctxtwop\valtwo}$ of the root cut.} Say that the hole falls inside $\val$ (the other cases are analogous), that is, $\mctx = \cuta{\pair{\lctxp\mctx^\bullet}{\lctxtwop\valtwo}}\mvartwo \mctxthreep{\para\mvartwo\var\vartwo \tmfour}$ for some $\mctx^\bullet$. The root step then writes as:
	\[\mctxfp\mvar = \cuta{\pair{\lctxp{\mctx^\bullet\ctxholep\mvar}}{\lctxtwop\valtwo}}\mvartwo \mctxthreep{\para\mvartwo\var\vartwo \tmfour}
 \rtotens  
 \mctxthreep{ \lctxp{\cuta{\mctx^\bullet\ctxholep\mvar}\var \lctxtwop{\cuta\valtwo\vartwo \tmfour}}}  = \tmtwo\]
	Then taking $\mctxtwo \defeq \mctxthreep{ \lctxp{\cuta{\mctx^\bullet}\var \lctxtwop{\cuta\valtwo\vartwo \tmfour}}}$ we have $\tmtwo = \mctxtwofp\mvar$, and
		\[\mctxfp\mval = \cuta{\pair{\lctxp{\mctx^\bullet\ctxholep\mval}}{\lctxtwop\valtwo}}\mvartwo \mctxthreep{\para\mvartwo\var\vartwo \tmfour}
 \rtotens  
 \mctxthreep{ \lctxp{\cuta{\mctx^\bullet\ctxholep\mval}\var \lctxtwop{\cuta\valtwo\vartwo \tmfour}}} = \mctxtwofp\mval\]

\emph{Moreover part}. It does not apply, because $\mctx$ is bad (having its hole inside a cut value).
	 
		\item \emph{The hole of $\mctx$ is in the right sub-term $\mctxthreep{\para\mvartwo\var\vartwo \tmfour}$ of the root cut}. Then $\mctx = \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo \mctxfour$ for some $\mctxfour$ such that $\mctxfourp\mvar=\mctxthreep{\para\mvartwo\var\vartwo \tmfour}$. Two sub-cases:
	\begin{enumerate}
	\item $\mctxthree\parallel\mctxfour$, then this case goes as sub-case $b$ of the $\rtoaxmone$ case (we are in case $(a)$), including the \emph{moreover} part.
	
	\item $\mctxthree\outer\mctxfour$. Therefore, $\mctxfour = \mctxthreep{\para\mvartwo\var\vartwo\mctx^\bullet}$ for some $\mctx^\bullet$. The root step then writes as:
	\[\mctxfp\mvar = \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo  \mctxthreep{\para\mvartwo\var\vartwo\mctx^\bullet\ctxholefp\mvar}  \rtotens  
	\mctxthreep{\lctxp{\cuta\val\var \lctxtwop{\cuta\valtwo\vartwo \mctx^\bullet\ctxholefp\mvar}}} = \tmtwo\]
	Then taking $\mctxtwo \defeq \mctxthreep{\lctxp{\cuta\val\var \lctxtwop{\cuta\valtwo\vartwo \mctx^\bullet}}}$ we have $\tmtwo = \mctxtwofp\mvar$, and
		\[\mctxfp\mval = \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo  \mctxthreep{\para\mvartwo\var\vartwo\mctx^\bullet\ctxholefp\mval}  \rtotens  
	\mctxthreep{\lctxp{\cuta\val\var \lctxtwop{\cuta\valtwo\vartwo \mctx^\bullet\ctxholefp\mval}}} = \mctxtwofp\mval\]
		
	\emph{Moreover part}. If $\ctx = \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo \mctxthree$ and $\mctx= \cuta{\pair{\lctxp\val}{\lctxtwop\valtwo}}\mvartwo \mctxthreep{\para\mvartwo\var\vartwo\mctx^\bullet}$ are good then $\mctxthreep{\para\mvartwo\var\vartwo\mctx^\bullet}$ is good and $\mvartwo\notin\dfv{\mctxthreep{\para\mvartwo\var\vartwo\mctx^\bullet}}$. Then  $\mctxtwo=\mctxthreep{\lctxp{\cuta\val\var \lctxtwop{\cuta\valtwo\vartwo \mctx^\bullet}}}$ is good and with the same dominating free variables by \reflemmap{good-stable-by-sub-ctx-rep}{par}. The step $\mctxfp\mval   \rtoaxmtwo   \mctxtwofp\mval$ has position $\ctx$, which is good by hypothesis.
	\end{enumerate}
\end{enumerate}

%%%%%%%%%%%
\item $\rtololli$. We have $\mctxfp\mvar = \cuta{\la\vartwo\tmthree}\mvar \mctxp{\suba\mvar\val\var \tmfour}
 \rtololli  
\mctxp{ \cuta\val\vartwo \lctxp{\cuta\valtwo\var \tmfour }}
 = \tmtwo$ with $\tmthree = \lctxp\valtwo$. As case $\rtotens$ using \reflemmap{good-stable-by-sub-ctx-rep}{sub} instead of \reflemmap{good-stable-by-sub-ctx-rep}{par}.
\end{itemize}
The exponential ones are:
\begin{itemize}
	%%%%%%%%%%%%%%%%%%
\item $\toess$.   We have $\mctxfp\mvar = \cuta{\exval} \evar \tmthree
 \rtoess 
\cutsub{\exval}\evar\tmthree = \tmtwo
$. By properness, $\exval$ cannot have free multiplicative variables, so the hole of $\mctx$ is in $\tmthree$ and we are in case $(a)$ and not in case $(b)$. We have $\mctx = \cuta{\exval} \evar\mctxthree$ with $\mctxthreefp\mvar = \tmthree$. The root step then writes as:
	\[\mctxfp\mvar = \cuta{\exval} \evar  \mctxthreefp\mvar
	\rtoess  
\cutsub{\exval} \evar  \mctxthreefp\mvar = (\cutsub{\exval} \evar  \mctxthree)\ctxholefp\mvar = \tmtwo\]
	Then taking $\mctxtwo \defeq \cutsub{\exval} \evar  \mctxthree$ we have $\tmtwo = \mctxtwofp\mvar$, and
		\[\mctxfp\mval = \cuta{\exval} \evar  \mctxthreefp\mval  
		\rtoess
	\cutsub{\exval} \evar  \mctxthreefp\mval = (\cutsub{\exval} \evar  \mctxthree)\ctxholefp\mval = \tmtwo = \mctxtwofp\mval\]



\emph{Moreover part}: it does apply, as goodness is only for micro steps.

%%%%%%%%%
\item $\rtoaxeone$.   We have $\mctxfp\mvar = \cuta{\exval} \evar \ctxtwofp{\evar}
 \rtoaxeone 
\cuta{\exval}\evar\ctxtwofp{\exval} = \tmtwo
$. By properness, $\exval$ cannot have free multiplicative variables, so the hole of $\mctx$ is in $\ctxtwo$ and we are in case $(a)$ and not in case $(b)$. The details go as for the corresponding case of $\rtoaxmone$.

%%%%%%%%%%%%%
	\item $\rtoaxetwo$.  We have $\mctxfp\mvar = \cuta{\evarthree}\evartwo\ctxtwop{\dera\evartwo\var \tmthree}
 \rtoaxetwo 
\cuta{\evarthree}\evartwo\ctxtwop{\dera\evarthree\var \tmthree} = \tmtwo$. The hole of $\mctx$ is necessarily in $\ctxtwo$ or $\tmthree$. Then we are in case $(a)$ and not in case $(b)$. The details go as for the corresponding case of $\rtoaxmtwo$.

%%%%%%%%%%%%%
	\item $\rtobder$.  We have $\mctxfp\mvar =  \cuta{\bang\tmthree}\evartwo\ctxtwop{\dera\evartwo\var \tmfour}
 \rtobder 
\cuta{\bang\tmthree}\evartwo\ctxtwo\ctxholep{\lctxp{\cuta\val\var \tmfour}}
 = \tmtwo$ with $\tmthree = \lctxp\val$.  By properness, $\tmthree$ cannot have free multiplicative variables, so the hole of $\mctx$ is in $\ctxtwop{\dera\evartwo\var \tmfour}$ and we are in case $(a)$ and not in case $(b)$. The details go as for the corresponding case of $\rtotens$, using \reflemmap{good-stable-by-sub-ctx-rep}{der} instead of \reflemmap{good-stable-by-sub-ctx-rep}{par}.

%%%%%%%%%%%%%
	\item $\rtow$.  We have $\mctxfp\mvar =  \cuta{\exval}\evartwo \tmthree
 \rtow  
\tmthree
 = \tmtwo$ with $\evartwo\notin\fv\tmthree$, and for which $\ctx=\ctxhole$. By properness, $\exval$ cannot have free multiplicative variables, so the hole of $\mctx$ is in $\tmthree$. Then we are in case $(a)$ and not in case $(b)$. We have $\mctx = \cuta{\exval} \evar\mctxthree$ with $\mctxthreefp\mvar = \tmthree$. Then taking $\mctxtwo \defeq \mctxthree$ we have $\tmtwo = \mctxtwofp\mvar$, and
		\[\mctxfp\mval = \cuta{\exval} \evar  \mctxthreefp\mval  
		\rtow
	  \mctxthreefp\mval = \mctxtwofp\mval\]

	\emph{Moreover part}. If $\ctx=\ctxhole$ and $\mctx = \cuta{\exval} \evar\mctxthree$ are good then $\mctxtwo \defeq \mctxthree$ is good and the position of the new step is still $\ctx$, which is good.
\end{itemize}
The inductive cases: 
\begin{itemize}
	%%%%%%%%%%%%%%%%%%
\item \emph{Cases with one sub-term (abstraction, promotion, par, dereliction)}. It follows from the \ih

\item \emph{Cases with two sub-terms (cut, tensor, subtraction)}. We treat the case of cut, the others are similar and simpler. Then $\mctxfp\mvar = \cuta\val\var\tmthree$. 
\begin{enumerate}
\item \emph{The rewriting step and the hole of $\mctx$ are in the same sub-term ($\val$ or $\tmthree$) of the root cut}. Then it follows from the \ih We detail the case in which they are both in $\tmthree$ in order to deal with the moreover part (which does not apply in the other case, as the step and the contextext are bad). Then $\ctx: \cuta\val\var\tmthree \Rew{a} \cuta\val\var\tmthree'$ with $\ctxthree:\tmthree \Rew{a} \tmthree'$, and $\mctx = \cuta\val\var\mctxthree$ with $\mctxthreep\mvar=\tmthree$. By \ih, there are two mutually exclusive cases:
\begin{enumerate}
\item there exists $\mctx^\bullet$ such that $\tmthree' = \mctx^\bullet\ctxholefp\mvar$ and a step $\ctx^\bullet_{\mval}:\mctxfp\mval \Rew{a} \mctxtwofp\mval$ for every $\mval$. Then we are in case $(a)$ by taking $\mctxtwo \defeq \cuta\val\var\mctx^\bullet$ and $\ctxtwo_{\mval} \defeq \cuta\val\var\ctx^\bullet_{\mval}$. 

	\emph{Moreover part}. If $\ctx=\ctxthree$ and $\mctx=\mctx^\bullet$ are good then $\ctxthree$ and $\mctxthree$ are good and $\var\notin\dfv{\ctxthree}$ and $\var\notin\dfv{\mctxthree}$. By \ih, $\mctx^\bullet$ is good and $\dfv{\mctxthree} = \dfv{\mctx^\bullet}$, and $\ctx^\bullet_{\mval}$ is good and $\dfv{\ctxthree} = \dfv{\ctx^\bullet_{\mval}}$. Then $\mctxtwo $ and $\ctxtwo_{\mval} $ are good and have the same dominating free variables of $\mctx$ and $\ctx$.
	
\item $\mctxthree = \mctx^\circ\ctxholep{\cuta\ctxhole\mvartwo\tmthree}$ for some 
$\mctx^\circ$ and $\ctxthree$ reduces the cut on $\mvartwo$. Then we are in case $(b)$ with $\mctxtwo \defeq \cuta\val\var\mctx^\circ\ctxholep{\cuta\ctxhole\mvartwo\tmthree}$. The \emph{moreover} part does not apply because $\mctx$ is bad.
\end{enumerate}


\item \emph{The rewriting step and the hole of $\mctx$ are not in the same sub-term ($\val$ or $\tmthree$) of the root cut}. We are in case $(a)$ and case $(b)$ does not hold. Similar to the previous case.
\end{enumerate}
\end{itemize}
	
	%%%%%%%%%%%%%%%%%%
	\item By induction on $\ctx: \mctxp{\tm_\mvar} \Rew{a} \tmtwo$, similar to \refpoint{aux-props-loc-confl-strong-comm-two}. Roughly, the multiplicative steps cannot touch $\tm_\mvar$ because they are linear and $\mctx$ does not capture $\mvar$ by hypothesis. The exponential steps cannot duplicate/erase $\tm_\mvar$ because it is in a $\mctx$ context, that is, the hole cannot be inside a $\bang$. 
		
	%%%%%%%%%%%%%%%%%%
	\item By induction on $\ctx: \mctxp{\para\mvar\var\vartwo \tm} \Rew{a} \tmtwo$, similar to \refpoint{aux-props-loc-confl-strong-comm-two}. Roughly, the multiplicative steps cannot touch $\para\mvar\var\vartwo $ because they are linear and $\mctx$ does not capture $\mvar$ by hypothesis. The exponential steps cannot duplicate/erase $\para\mvar\var\vartwo $ because it is in a $\mctx$ context, that is, the hole cannot be inside a $\bang$. The part about $\ctxthree$ is simply due to the \emph{at a distance} or \emph{contextual} nature of the rules.
	
	\item As in the previous point, with the slight complication that subtractions have two sub-terms $\val$ and $\tmfour$, which give the more involved statement, but the reasoning is the same.
	
	%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\item By induction on the step $\ctx:\ctxtwofp\evar \Rew{a} \tmtwo$, similar to \refpoint{aux-props-loc-confl-strong-comm-two}.

%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\item By induction on the step $\ctx:\ctxtwop{\dera\evar\var\tmthree} \Rew{a} \tmtwo$, similar to \refpoint{aux-props-loc-confl-strong-comm-two}.

\end{enumerate}
\end{proof}

